Mix $\star$-autonomous quantales and the continuous weak order

The set of permutations on a finite set can be given a lattice structure (known as the weak Bruhat order). The lattice structure is generalized to the set of words on a fixed alphabet $\Sigma = \{ x, y, z, ... \}$, where each letter has a fixed number of occurrences (these lattices are known as multinomial lattices and, in dimension 2, as lattices of lattice paths). By interpreting the letters $x, y, z, ...$ as axes, these words can be interpreted as discrete increasing paths on a grid of a $d$-dimensional cube, where $d = {\rm card}(\Sigma)$. We show in this paper how to extend this order to images of continuous monotone paths from the unit interval to a $d$-dimensional cube. The key tool used to realize this construction is the quantale $\mathsf{L}_{\vee}(\mathbb{I})$ of join-continuous functions from the unit interval to itself; the construction relies on a few algebraic properties of this quantale: it is $\star$-autonomous and it satisfies the mix rule. We begin developing a structural theory of these lattices by characterizing join-irreducible elements, and by proving these lattices are generated from their join-irreducible elements under infinite joins.

==> macros.tex <==
\RequirePackage{ifthen}
\newcommand{\nollncs}[1]{\ifthenelse{\isundefined{\llncs}}{#1}{}}
\newcommand{\onlyllncs}[1]{\ifthenelse{\isundefined{\llncs}}{}{#1}}

\RequirePackage{amsmath,amssymb}
\newcommand{\tand}{\text{ and }}
\newcommand{\tiff}{\text{ iff }}
\newcommand{\toth}{\text{ otherwise }}
\RequirePackage{txfonts}
\RequirePackage{tikz-cd}
\RequirePackage{wrapfig}

\RequirePackage{comment}
\excludecomment{toappendix}

\newenvironment{prop}{\vskip 6pt\par\noindent{\bf Proposition.~\em}}{\par\vskip 6pt}

\newenvironment{thm}{\vskip 6pt\par\noindent{\bf Theorem.~\em}}{\par\vskip 6pt}

\nollncs{
  \RequirePackage{amsthm}
  \newtheorem{theorem}{Theorem}
  \newtheorem{proposition}{Proposition}
  \newtheorem{lemma}{Lemma}
  \newtheorem{corollary}{Corollary}
  \theoremstyle{definition}
  \newtheorem{definition}{Definition}
  \theoremstyle{remark}
  \newtheorem{remark}{Remark}
  \newtheorem{example}{Example}
}


\RequirePackage{xspace}
\newcommand{\staraut}{$\star$-autonomous\xspace}
\newcommand{\saq}{\staraut quantale\xspace}
\newcommand{\msaq}{mix \staraut quantale\xspace}
\newcommand{\U}[1]{\mid#1\mid}
\newcommand{\opp}[1]{{#1}^{\star}}
\newcommand{\Opp}[1]{#1^{\star}}
\newcommand{\opprj}[1]{\Joinof{\Radj{#1}}}
\newcommand{\oppml}[1]{\Ladj{\Meetof{#1}}}
\newcommand{\Star}[1]{{#1}^{\star}}

\newcommand{\oppopp}[1]{{#1}^{\star\star}}
\newcommand{\oppfun}{\opp{(-)}}
\newcommand{\secRef}[1]{Section~\ref{sec:#1}}

\newcommand{\Q}{\mathbb{Q}}
\newcommand{\qQ}{Q}

\newcommand{\N}{\mathbb{N}}
\newcommand{\I}{\mathbb{I}}

\renewcommand{\L}{\mathsf{L}}
\newcommand{\LI}[1][]{\L(\I^{#1})}
\newcommand{\LId}{\LI[d]}
\newcommand{\Lj}{\L_{\vee}}
\newcommand{\Lf}{\L_{\mathfrak{f}}}
\newcommand{\LfI}{\Lf(\I)}
\newcommand{\LfId}{\Lf(\I^{d})}
\newcommand{\LjI}{\L_{\vee}(\I)}
\newcommand{\LmI}{\L_{\land}(\I)}
\newcommand{\meetof}[1]{{#1}^{\land}}
\newcommand{\joinof}[1]{{#1}^{\vee}}
\newcommand{\meetofjoinof}[1]{{#1}^{\vee\land}}
\newcommand{\joinofmeetof}[1]{{#1}^{\land\vee}}

\newcommand{\Meetof}[1]{#1^{\land}}
\newcommand{\MeetOf}[1]{\Meetof{#1}}
\newcommand{\Joinof}[1]{#1^{\vee}}

\newcommand{\ladj}[1]{{#1}_{\ell}}
\newcommand{\radj}[1]{{#1}_{\rho}}
\newcommand{\Ladj}[1]{#1_{\ell}}
\newcommand{\Radj}[1]{#1_{\rho}}

\newcommand{\continuous}{continuous\xspace}
\newcommand{\jcont}{join-\continuous}
\newcommand{\jc}{\jcont}
\newcommand{\mcont}{meet-\continuous}
\newcommand{\mc}{\mcont}
\newcommand{\bcont}{bi-\continuous}
\newcommand{\bc}{\bcont}
\newcommand{\tcont}{topologically \continuous}

\newcommand{\rto}{\xrightarrow{\;\;}}
\newcommand{\rTo}{\rto}
\newcommand{\lrimpl}{\multimap}
\newcommand{\rlimpl}{\multimapinv}

\newcommand{\prodd}[2][d]{{#2}^{\couples{#1}}}
\newcommand{\PrLQ}{\prodd{Q}}
\newcommand{\PrdQ}{\prodd{Q}}
\newcommand{\PrLI}[1][d]{\prodd[#1]{\LjI}}


\newcommand{\closure}[1]{\overline{#1}}
\newcommand{\cl}[1]{\closure{#1}}
\newcommand{\interior}[1]{#1^{\circ}}
\renewcommand{\int}[1]{\interior{#1}}
\newcommand{\set}[1]{\{\,#1\,\}}
\newcommand{\two}{{\bf 2}}
\newcommand{\Ld}[2][d]{\L_{#1}(#2)}

\newcommand{\Id}[1][d]{\I^{d}}
\newcommand{\p}{\mathsf{p}}
\newcommand{\IQ}{\I \cap \mathbb{Q}}
\newcommand{\card}{\mathrm{card}}

\newcommand{\couples}[1]{\setof{#1}_{2}}
\newcommand{\cd}{\couples{d}}
\newcommand{\lin}[1]{To be defined}
\newcommand{\setof}[1]{[#1]}
\newcommand{\osf}{one step function\xspace}
\newcommand{\ji}[1]{e_{#1}}
\newcommand{\mi}[1]{m_{#1}}
\newcommand{\Ji}[1]{\MeetOf{\ji{#1}}}
\newcommand{\JI}[1]{E_{#1}}
\newcommand{\jp}{join-prime\xspace}
\newcommand{\cjp}{completely \jp}
\newcommand{\jirr}{join-irreducible\xspace}
\newcommand{\mirr}{meet-irreducible\xspace}
\newcommand{\Mirr}{Meet-irreducible\xspace}
\newcommand{\cjirr}{completely \jirr}
\newcommand{\Fam}[1]{\langle \,#1 \,\rangle}
\newcommand{\mji}{\mu^{\vee}}
\newcommand{\Mji}{M^{\vee}}
\newcommand{\dimmi}{\dim^{\land}}
\newcommand{\dimji}{\dim^{\vee}}
\newcommand{\mmi}{\mu^{\land}}
\newcommand{\Mmi}{M^{\land}}
\newcommand{\Mi}[4]{M^{#3,#4}_{#1,#2}}
\newcommand{\JJi}[4]{E^{#3,#4}_{#1,#2}}


\newcommand{\eofclaim}{\hfill{\it Claim}~\qed\par}
\newcommand{\LADJ}{left adjoint\xspace}
\newcommand{\RADJ}{right adjoint\xspace}
\newcommand{\resp}{resp.,\xspace}
\newcommand{\covered}{\prec}
\newcommand{\wBo}{weak Bruhat order\xspace}
\newcommand{\wo}{weak order\xspace}
\newcommand{\cwBo}{continuous \wBo}
\newcommand{\cwo}{continuous \wo}

\newcommand{\DMNc}{Dedekind-MacNeille completion\xspace}
\newcommand{\appr}[1][v]{\mathtt{appr}_{#1}}

\newcommand{\Associahedra}{associahedra\xspace}
\newcommand{\Permutohedra}{permutohedra\xspace}
\newcommand{\Permutohedron}{permutohedron\xspace}


